Capturing Quantum Snapshots from a Single Copy via Mid-Circuit Measurement and Dynamic Circuit

We propose Quantum Snapshot with Dynamic Circuit (QSDC), a hardware-agnostic, learning-driven framework for capturing quantum snapshots: non-destructive estimates of quantum states at arbitrary points within a quantum circuit, which can then be classically stored and later reconstructed. This functionality is vital for introspection, debugging, and memory in quantum systems, yet remains fundamentally constrained by the no-cloning theorem and the destructive nature of measurement. QSDC introduces a guess-and-check methodology in which a classical model, powered by either gradient-based neural networks or gradient-free evolutionary strategie, is trained to reconstruct an unknown quantum state using fidelity from the SWAP test as the sole feedback signal. Our approach supports single-copy, mid-circuit state reconstruction, assuming hardware with dynamic circuit support and sufficient coherence time. We validate core components of QSDC both in simulation and on IBM quantum hardware. In noiseless settings, our models achieve average fidelity up to 0.999 across 100 random quantum states; on real devices, we accurately reconstruct known single-qubit states (e.g., Hadamard) within three optimization steps.

==> Abstract_memory_bank.tex <==
One of the central challenges in quantum computing arises from wavefunction collapse during measurement. To determine a quantum state, traditional methods such as Quantum State Tomography (QST) require a series of destructive measurements on multiple copies of the state, ultimately erasing the very state we seek to understand. In this work, we introduce a novel \texttt{Quantum Memory Bank Architecture} that enables the observation of quantum states without directly measuring, and thereby destroying them. 
% 
Our architecture enables the observation of multiple quantum states at different points within a single circuit, allowing them to be saved \texttt{(`deposited')} into a classical memory without direct measurement or destruction. These states can then be accessed \texttt{(`withdrawn')} on demand by downstream applications during execution, introducing a dynamic and programmable notion of quantum memory that supports modular, non-destructive quantum workflows.

We leverage the SWAP test to compute fidelity between an unknown state and a generated estimate to guide both gradient-based and gradient-free optimization strategies to recover the state vector or density matrix from a single copy of the unknown state, using mid-circuit measurement techniques.
% 
A neural network is trained to generate high-fidelity approximations of the unknown state by observing only the ancilla qubit from the SWAP test. It learns to associate changes in its inputs with resulting fidelity scores, allowing it to converge on the correct state. We use state vector and unitary-based techniques to reconstruct pure states, and extend the method to mixed states using density matrix formalism.
% 
Our approach achieves fidelity $\sim 1.0$ for Hadamard states on real IBM superconducting qubit hardware, and an average fidelity of $0.999$ across 1000 random states in simulation. The architecture is hardware-agnostic and applicable to any quantum computing platform. Unlike traditional QST methods, our approach allows single-copy, mid-circuit recovery of quantum states with fidelity $\sim 1.0$ using hardware-validated techniques.
%The codebase is available here \url{https://github.com/DebarshiKunduPSU/NMQST}.    


% Traditional Quantum state tomography (QST) is the process of obtaining a complete description of a quantum system by performing measurements on a set of informationally complete observables and in the process destroying (due to measurement) the original unknown states. 
% We propose a Quantum State Tomography (QST) method without measuring (destroying) the original unknown state using both gradient-based and gradient-free methods for estimating the state vector and density matrix of an unknown quantum state. Our approach leverages the SWAP test to compute fidelity and uses this information to guide the estimation process. By performing multiple SWAP tests within the decoherence time of the unknown state's qubits, our method enables quantum state tomography using only a single copy of the unknown state. 
% We employ a neural network model that iteratively learns to generate the correct state vector or density matrix by measuring only the ancilla qubit. The network learns to associate changes in the input with changes in fidelity, allowing it to generate states with high fidelity. Our method achieves fidelity 1 on real quantum hardware for Hadamard states, and an average fidelity of 0.999 for 1000 random states in simulation.

% This approach introduces a novel paradigm in QST that does not require target unknown states to be measured/destroyed and able to dynamically estimate the unknown state. This opens up new possibilities for algorithm development in dynamic circuits.  The process is hardware-agnostic and feasible for implementation on any quantum computing platform. We demonstrate our results using IBM’s superconducting qubit-based quantum computers. We also demonstrate our method leads to quantum memory because it enables dynamically estimating states and therefore saving the snapshots classically which can be retrieved anytime using quantum memory during dynamic circuit execution. 
% The codebase is available here \url{https://github.com/DebarshiKunduPSU/NMQST}

% Quantum state tomography (QST) is the process of obtaining a complete description of a quantum system by performing measurements on a set of informationally complete observables. However, traditional QST methods require an exponential number of measurements as the system size increases, making them impractical for large-scale quantum systems. QST involves estimating the density matrix of an unknown quantum state through repeated measurements, assuming that the source consistently produces identical copies of the state. 
% However, the assumption of access to multiple identical copies is often unrealistic, particularly in the NISQ (Noisy Intermediate-Scale Quantum) era. 
% In this work, we propose \hl{I think you should start with NN model that is trained using swap test. Right now its all mixed up-- both gradient-based and gradient-free methods for estimating the state vector and density matrix of an unknown quantum state without destroying the original state. Our approach leverages the SWAP test to compute fidelity and uses this information to guide the estimation process. By performing multiple SWAP tests within the decoherence time of the unknown state's qubits, our method enables quantum state tomography using only a single copy of the unknown state. 

% We employ a neural network model that iteratively learns to generate the correct state vector or density matrix by measuring only the ancilla qubit. The network learns to associate changes in the input with changes in fidelity, allowing it to generate states with high fidelity. Our method achieves fidelity 1 on real quantum hardware for Bell states, and an average fidelity of 0.999 for 1000 random states in simulation.

% This approach introduces a novel paradigm in QST that is hardware-agnostic and feasible for implementation on any quantum computing platform. We demonstrate our results using IBM’s superconducting qubit-based quantum computers, which were freely accessible for this work.}

%version 2
% Quantum mechanics imposes a fundamental limitation on observing a system without disturbing its state, complicating the study and control of quantum systems. While quantum state tomography provides a method for reconstructing states through repeated measurements, its destructive nature makes it impractical for larger quantum systems. In this work, we explore a novel approach to reconstruct unknown quantum states using classical machine learning techniques. We propose three primary methods: the first estimates the state using a state vector, the second utilizes a unitary representation, and the third employs a density matrix, with the latter capable of reconstructing both pure and mixed states. Each method leverages a classical neural network to achieve accurate state estimation. \hl{need to add results}
% Although our approach requires classical resources that scale exponentially with the number of qubits ($2^n$ complexity) — a well-known challenge in state reconstruction — this remains feasible for the small-scale circuits typical of the NISQ (Noisy Intermediate-Scale Quantum) era. 



% version 1
% Until more efficient quantum information storage techniques are developed, our method offers a practical solution for near-term quantum memory applications, providing a non-invasive means of accessing state information without direct measurement.

% Can we store Quantum State information classically? We answer the question in this work. We propose a method to figure out an unknown Quantum State with a classical machine learning approach. Although the proposed method needs $2^n$ complexity of classical resources to store quantum state (unsurprisingly ), we have shown this approach is suitable for NISQ era small Qubits until a better method to store quantum information is figured out. 

==> memory_bank_tex/application_memory_bank.tex <==
\subsection{Quantum State Tomography}
Measurement comparison with QST technology

\subsubsection{Background: What is Quantum State Tomography (QST)?}

Quantum State Tomography (QST) is the process of reconstructing a quantum state $\rho$ from a complete set of measurement outcomes. For a pure state $\ket{\psi} \in \mathbb{C}^{2^n}$, QST involves performing measurements in multiple bases, collecting statistics over repeated experiments, and solving an inverse problem (e.g., via maximum likelihood estimation or convex optimization) to recover the state.

\vspace{1ex}
\noindent
However, QST suffers from several major bottlenecks:
\vspace{-0.5ex}
\begin{itemize}
  \setlength\itemsep{0.2em}
  \item \textbf{Exponential scaling:} The number of required measurements grows exponentially with the number of qubits: at least $\mathcal{O}(4^n)$ parameters are needed to describe a general mixed state.
  \item \textbf{Measurement overhead:} A full set of tomographic measurements must be performed in all combinations of Pauli bases.
  \item \textbf{Post-processing complexity:} Reconstructing the density matrix or pure state involves solving a high-dimensional inverse problem.
  \item \textbf{Noise sensitivity:} Measurement errors and statistical fluctuations can significantly degrade reconstruction fidelity.
\end{itemize}

\vspace{1ex}
\noindent
\textbf{Advantages of Our Method:} Our proposed method replaces the measurement-heavy QST pipeline with a learning-based approach, which optimizes a neural model to generate the unknown state by directly maximizing fidelity via quantum circuits (e.g., the swap test). Below are detailed comparisons across key dimensions in Table \ref{table1}

% \begin{table*}[h!]\label{table1}
% \centering
% \caption{Comparison between Traditional Quantum State Tomography and Our Fidelity-Based Learning Method}
% \begin{tabular}{|p{2cm}|p{7cm}|p{7cm}|}
% \hline
% \textbf{Feature} & \textbf{Traditional Quantum State Tomography} & \textbf{Our Fidelity-Based Learning Method} \\
% \hline
% \textbf{Measurement Complexity} & Requires $O(3^n)$ measurement settings across multiple bases (X, Y, Z) & Requires only one observable (Pauli-Z on control qubit in swap test) \\
% \hline
% \textbf{Scalability with Qubits} & Poor scalability due to exponential growth in measurements and reconstruction complexity & Good scalability; uses $2n+1$ qubits in swap test and avoids exponential post-processing \\
% \hline
% \textbf{Noise Robustness} & Sensitive to SPAM errors and statistical noise; requires regularization & Robust to noise via iterative optimization and fidelity smoothing \\
% \hline
% \textbf{Training Feedback} & Passive; all data collected before reconstruction & Active; model receives fidelity-based feedback each iteration \\
% \hline
% \textbf{Computational Overhead} & High classical cost for density matrix estimation or MLE & Minimal; no post-processing, output is directly learned \\
% \hline
% \textbf{Generalization Capability} & None; each state treated independently & Can generalize across families of states if trained appropriately \\
% \hline
% \textbf{Data Reusability} & No reuse of measurements once collected & Training inherently reuses data via backpropagation \\
% \hline
% \textbf{Best Use Case} & Full tomography of low-qubit mixed states & Pure or low-rank states where fidelity is sufficient \\
% \hline
% \end{tabular}
% \end{table*}

% \subsection{Mid Circuit Measurement, Snapshot}


\subsection{Application to Mid-Circuit Measurement and Quantum Snapshots}

As quantum hardware evolves, mid-circuit measurements (MCM) and quantum snapshots are becoming essential tools for enabling feedback-based computation, error detection, adaptive protocols, and time-evolving state tracking. These operations allow partial access to the state of a quantum system during the course of a computation, without collapsing the entire wavefunction.

Our proposed method---reconstructing quantum states using a neural generator trained via the swap test---offers unique benefits in both these contexts.

\subsubsection{Quantum Snapshot Reconstruction}

A quantum snapshot refers to a partial or complete capture of the state of a quantum system at an intermediate point in a quantum circuit. This is often used for:
\begin{itemize}
    \item Debugging and circuit introspection
    \item Tracking state evolution in time-dependent processes
    \item Verifying the correctness of variational protocols
\end{itemize}

However, in practical devices, taking full snapshots (via tomography) is infeasible due to resource costs.

\paragraph{How Our Method Helps} Given access to the quantum state at an intermediate point in the circuit (e.g., via a saved vector or partial tomography), we can train a generator model to replicate that snapshot.

Using our swap-test-based fidelity loss, the generator can be optimized to recreate the snapshot state without requiring repeated destructive measurements.

Once trained, this generator acts as a compact, reusable representation of the intermediate quantum state, useful for debugging, state injection, or later analysis.

This avoids the cost of storing large state vectors and instead provides a learned, parameter-efficient encoding of the state at that point in the circuit.

\subsubsection{Mid-Circuit Measurement and Adaptive State Tracking}

Mid-circuit measurements allow specific qubits to be measured during computation and then reused or modified conditionally, enabling:
\begin{itemize}
    \item Error mitigation and detection
    \item Adaptive measurement strategies
    \item Measurement-based quantum computation
\end{itemize}

However, these measurements can disrupt the remaining quantum state, and their outcomes are often stochastic. In such settings, learning to predict or approximate the post-measurement state becomes important.

\paragraph{How Our Method Helps} Suppose a mid-circuit measurement is made on a subset of qubits, collapsing the state to a known branch conditioned on the measurement result.

The remaining unmeasured qubits are in a projected (but unknown) state.

Our method can reconstruct this projected post-measurement state by treating it as the new unknown 
\(|\psi\rangle\), and learning a generator that replicates it with high fidelity.

This is particularly useful in:
\begin{itemize}
    \item Quantum simulations, where adaptive branching occurs
    \item Error decoding, where one wants to learn the most probable state after syndrome measurement
    \item Quantum control, where the system evolves depending on feedback and state collapse
\end{itemize}

Moreover, since mid-circuit measurement often involves conditional operations, we can treat the measurement outcome as a condition \(z\), and train a conditional generator \(G(z)\) that learns to generate the correct projected state based on classical measurement history.







\subsection{Circuit Optimization}
\subsection{Quantum Repeater}
\subsection{Quantum Sensor}

==> memory_bank_tex/results_memory_bank.tex <==
We have tested our hypothesis in real hardware (IBM Superconducting qubits), noisy simulations using IBM hardware noise models, and noiseless simulations using AerSimulator in Pennylane. 

% Due to lack of resources in real hardware we have verified few 1 qubit known states such as states |0> = [1, 0], |1> = [0, 1], Bell State = 1/ \sqrt{2}[1,1] and we achieved fidelity of 1 within 3 epochs. 
Due to lack of resources on real hardware, we have verified a few known single-qubit states, such as the states $\ket{0} = [1, 0]$, $\ket{1} = [0, 1]$, and the Hadamard state $\frac{1}{\sqrt{2}}[1, 1]$. We achieved a fidelity of $1$ within $3$ epochs.

We have executed extensive experiments using both noisy and noiseless simulation which results are presented below. 
\input{results_noisemodel_memory_bank}

\subsection{Noisy and Noiseless Simulation Experiments}
\subsubsection{Distribution between Target and Reconstructed State Fidelity}
\ref{fig:statevector_unitary_fidelity_distribution} shows fidelity values as per \ref{fidelity}. The fidelity was calculated by randomly sampling 1000 states, and then the corresponding fidelity was reported from the noiseless simulation using the Qiskit AerSimulator. The results show that the min fidelity achieved is 99.9\% which is much better than the SOTA method 99.1 \% \cite{liu_variational_2020} and it is achieved much faster within 30 epochs. (some of them reached to best fidelity much earlier and we did early stopping for those cases.  ) 
\hl{TBD: Plot qubit vs epoch needed and time needed}
% \begin{figure}[]
%     \centering
%     \includegraphics[width=1\linewidth]{fig/statevector_unitary_fidelity_distribution.pdf}
%     \caption{Statevector unitary fidelity distribution}
%     \label{fig:statevector_unitary_fidelity_distribution}
% \end{figure}

% Here is a comparison table across various literature and our work.

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|c|c|c|}
% \hline
% \textbf{Metric} & \textbf{Our Approach} & \textbf{Liu et al.} & \textbf{Paper 3} \\
% \hline
% Min Fidelity Achieved & 99.9\% & 99.1\% & -- \\
% \hline
% Epochs & 30 (max) & -- & -- \\
% \hline
% Number of Shots & -- & -- & -- \\
% \hline
% Noisy Sim Fidelity & -- & X & X \\
% \hline
% Noisy Sim Epochs & -- & X & X \\
% \hline
% Noisy Sim Shots & -- & X & X \\
% \hline
% Hardware Results & Yes & No & No \\
% \hline
% \end{tabular}
% \caption{Comparison of Quantum State Reconstruction Results Across Papers}
% \label{tab:paper_comparison}
% \end{table}


Find the 6-sigma value and other stat values
\subsubsection{Amplitude Comparison of Target and Reconstructed States }
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/amplitude_3d_plot.pdf}
    \caption{Amplitude Comparison of Target and Reconstructed States}
    \label{fig:amplitude_3d_plot}
\end{figure}
We have picked a couple of states to show that amplitude probabilities in 2 qubit basis states are almost same which reiterates the fact fidelity is high and also the right measure to compare similarity between quantum states. 
\subsubsection{Entanglement Quality of Target and Reconstructed States }
In order to determine whether our unknown target states are sufficiently entangled, we measured the entanglement entropy of those states using the following method. We calculated the von Neumann entropy of the reduced density matrix obtained by performing a bipartition of the system. Specifically, for a given pure state $\lvert\psi\rangle$, we traced out half of the system to obtain the reduced density matrix $\rho_A = \mathrm{Tr}_B(\lvert\psi\rangle\langle\psi\rvert)$, and then computed the entanglement entropy as
\[
S(\rho_A) = -\mathrm{Tr}(\rho_A \log \rho_A).
\]
This entropy quantifies how entangled a state is across the chosen bipartition.

We observed a good mixture of highly entangled states and matrix product states with low entanglement. Notably, the reconstructed states exhibited entanglement properties closely matching those of the corresponding unknown target states. This confirms the robustness of our method across a range of entangled and weakly entangled (matrix product) states. Figure~4 (left) displays the entanglement entropy of the target states, while Figure~4 (right) demonstrates that the entanglement entropy of the generated states aligns well with that of the target states. This strong agreement further supports that the generated states faithfully capture the entanglement structure of the target states.

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/statevector_entanglement_entropy.pdf}
    \caption{Statevector entanglement entropy}
    \label{fig:statevector_entanglement_entropy}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/statevector_fidelity_distribution.pdf}
    \caption{Statevector fidelity distribution}
    \label{fig:statevector_fidelity_distribution}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/unitary_fidelity_distribution.pdf}
    \caption{Unitary fidelity distribution}
    \label{fig:unitary_fidelity_distribution}
\end{figure}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/density_matrix_fidelity_distribution.pdf}
    \caption{Density matrix with fidelity and ulhman fidelity}
    \label{fig:density_matrix_fidelity_distribution}
\end{figure}

\subsubsection{Calculation of total number of shots/copy}
\subsubsection{Transferability of Model}
We explored the pretraining of models by initially training a single model on 1000 randomly generated quantum states. This pre-trained model was then evaluated on a separate set of 100 unknown and known quantum states, as summarized in Table~\ref{tab:quantum_state_result}. We observed an average improvement of approximately $70\%$ in the number of epochs required to reach a comparable fidelity.

\subsection{Comparison}

\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{fig/grouped_barplot_correct_order.pdf}
    \caption{State Vector}
    \label{fig:grouped_barplot_correct_order}
\end{figure}

\input{table_master_results}
\input{table_big_state}























==> memory_bank_tex/results_noisemodel_memory_bank.tex <==
\subsection{Noisemodel}
% \subsection*{Noise Model Specification}

% To emulate the behavior of near-term quantum devices, we incorporate a customized noise model based on Qiskit's \texttt{NoiseModel} framework. This model captures both gate-dependent and qubit-specific imperfections, enabling the simulation of quantum circuits under realistic conditions. The key properties of the noise model are as follows:

% \begin{itemize}
%     \item \textbf{Supported Gate Set}: The noise model operates over the following basis gates:
%     \[
%     \{\texttt{cx},\ \texttt{delay},\ \texttt{id},\ \texttt{measure},\ \texttt{reset},\ \texttt{rz},\ \texttt{sx},\ \texttt{x}\}
%     \]
%     These include both native quantum operations and auxiliary operations such as idle and measurement.

%     \item \textbf{Noisy Operations}: Noise is explicitly modeled for a subset of these gates:
%     \[
%     \{\texttt{id},\ \texttt{cx},\ \texttt{x},\ \texttt{measure},\ \texttt{sx}\}
%     \]
%     This implies that these operations incur gate-specific decoherence or stochastic errors.

%     \item \textbf{Noisy Qubits}: The model includes noise on all physical qubits. Each qubit is subject to noise depending on the operation applied.

%     \item \textbf{Instruction-Specific Noise Mapping}: The noise model specifies fine-grained gate-qubit combinations. For instance:
%     \begin{itemize}
%         \item Two-qubit errors are defined for \texttt{cx} gates between all pairwise combinations, such as \texttt{cx}(0,1), \texttt{cx}(2,3), etc., to simulate entangling gate infidelities.
%         \item Single-qubit noise affects identity operations (\texttt{id}) to model \textit{idle decoherence}, as well as gates like \texttt{x}, \texttt{sx}, and \texttt{measure} to simulate \textit{unitary errors} and \textit{readout noise}.
%     \end{itemize}
% \end{itemize}



% \subsection*{Impact on Quantum State Reconstruction}

% In our setting, this noise model plays a crucial role in evaluating the quality of reconstructed quantum states. Specifically, it impacts:
% \begin{itemize}
%     \item \textbf{State preparation circuits}, used by the generative model to produce candidate quantum states;
%     \item \textbf{Fidelity estimation via the swap test}, which acts as the primary loss function;
%     \item \textbf{Gradient-based training routines}, where parameter updates must remain robust to statistical fluctuations introduced by noise.
% \end{itemize}

% By incorporating this detailed noise structure, our learning framework becomes both device-aware and resilient to hardware-induced infidelities, facilitating accurate and transferable quantum state reconstruction in the NISQ regime.

% 


To realistically simulate the behavior of near-term noisy quantum processors, we incorporate a detailed gate-level noise model derived from an IBM GenericBackendV2 for the required number of qubits. This model is integrated using Qiskit's \texttt{NoiseModel} interface and imported into PennyLane via a custom Aer device. The key features of the model are outlined below:

\begin{itemize}
    \item \textbf{Basis Gate Set}: The noise model supports the following native operations:
    \[
    \{\texttt{cx},\ \texttt{delay},\ \texttt{id},\ \texttt{measure},\ \texttt{reset},\ \texttt{rz},\ \texttt{sx},\ \texttt{x}\}
    \]
    
    \item \textbf{Noisy Instructions}: Noise is defined on a subset of these operations:
    \[
    \{\texttt{id},\ \texttt{cx},\ \texttt{sx},\ \texttt{x},\ \texttt{measure}\}
    \]
    indicating that idle operations, single-qubit unitaries, and two-qubit entangling gates are all subject to non-trivial noise processes.

    \item \textbf{Qubits with Noise}: All qubits indexed as \( q_0, q_1, q_2, q_3 ... q_n \) are affected by gate-dependent noise.

    \item \textbf{Gate-Qubit Error Map}: The noise model provides fine-grained control over qubit-specific gate errors via \texttt{QubitChannel} representations. These channels internally encode Kraus operators to simulate stochastic quantum noise. For instance:
    \begin{itemize}
        \item CNOT gates between qubit pairs exhibit asymmetric noise profiles. For example:
        \begin{itemize}
            \item \texttt{cx}(0,1): \texttt{QubitChannel} with 16 Kraus operators
            \item \texttt{cx}(0,2): \texttt{QubitChannel} with 9 Kraus operators
        \end{itemize}
        \item Single-qubit gates such as \texttt{id}, \texttt{sx}, and \texttt{x} apply noisy channels using 3 to 4 Kraus operators.
    \end{itemize}

    \item \textbf{Asymmetric Noise Modeling}: The number of Kraus operators varies across different gates and qubit pairs, reflecting real device asymmetries in gate infidelity. This captures not only gate-dependent but also hardware-layout-specific noise behavior.
    
    % \item \textbf{Readout Noise Warning}: While the noise model includes readout noise channels for \texttt{measure} operations, current limitations in PennyLane's Qiskit interface result in these channels being skipped during simulation:
    % \begin{quote}
    % \texttt{UserWarning: Readout errors are not supported currently and will be skipped.}
    % \end{quote}
    % Therefore, measurement errors are not simulated explicitly.
\end{itemize}

This nuanced noise model enables us to perform variational training and quantum state reconstruction under physically realistic conditions. By introducing non-uniformity in fidelity degradation across gates and qubit pairs, the model better represents the noise anisotropy observed in superconducting qubit architectures. It thus provides a critical tool for benchmarking algorithmic robustness, especially when optimizing under the fidelity loss metric derived from the swap test.

In Table~\ref{tab:noisemodel}, we provide a summary of the noise model corresponding to a 5-qubit quantum circuit, adapted from an IBM 5-qubit quantum backend. This configuration reflects a dense interaction topology and non-trivial noise distribution, characteristic of real IBMQ processors such as \texttt{ibmq\_quito} or \texttt{ibmq\_lima}. It enables us to assess the performance of quantum algorithms under realistic, gate-dependent, and correlated noise conditions.

\begin{table*}[h!]
\centering
\caption{5 Qubit Qiskit Noise Model Summary}
\begin{tabular}{c|c|c}

\textbf{Gate Type} & \textbf{Qubits Affected} & \textbf{Noise Description} \\
\hline \hline
\texttt{id}       & $q_0, q_1, q_2, q_3, q_4$ & Idle decoherence \\ \hline
\texttt{x}        & $q_0, q_1, q_2, q_3, q_4$ & Bit-flip or unitary gate noise \\ \hline
\texttt{sx}       & $q_0, q_1, q_2, q_3, q_4$ & Under/over-rotation errors \\ \hline
\texttt{measure}  & $q_0, q_1, q_2, q_3, q_4$ & Readout error (bit-flip) \\ \hline
\texttt{cx}       & All pairs of 2-qubit combinations among $q_0$–$q_4$ & Entangling gate noise \\
\hline \hline
\end{tabular}
\label{tab:noisemodel}
\end{table*}

==> methods_snapshot_short.tex <==
\subsection{QSDC Framework and Setup}
We propose a framework to estimate an unknown quantum state at arbitrary points within a quantum circuit and store it classically for later retrieval. QSDC operates in a hybrid quantum-classical loop, where a classical controller iteratively updates a candidate quantum state based on fidelity measurements. This process assumes sufficiently long decoherence times to allow for mid-circuit resets, fidelity evaluation, and model updates within the coherence window.

The unknown quantum state is assumed to be available as a circuit-level representation, a valid abstraction for modern quantum hardware. For demonstration, we generate target states using PennyLane’s \texttt{StatePrep}. A candidate state is initialized by a classical model and re-prepared in the circuit. A SWAP test with an ancilla qubit evaluates fidelity, which serves as feedback to iteratively refine the candidate state.

We consider three representations of quantum states: (i) state vectors for pure states, (ii) density matrices for mixed and pure states, and (iii) unitaries that prepare the state from $\ket{0}^{\otimes n}$. Each representation is learned using either a gradient-based or gradient-free method, as described below.

\subsection{Common Estimation Procedure}

At each training step:
\begin{enumerate}
    \item A candidate quantum state $\ket{\psi}$ is generated.
    \item The fidelity $F = |\braket{\psi | \phi_u}|^2$ is estimated via a SWAP test with the unknown state $\ket{\phi_u}$.
    \item The candidate is refined using either gradient descent (via backpropagation) or evolutionary updates.
\end{enumerate}

\textbf{Fidelity Computation via SWAP Test:}
Given states $\ket{\psi}$ and $\ket{\phi_u}$, fidelity is evaluated as $F = \langle Z \rangle$ on the ancilla qubit in a SWAP test circuit. For $2n+1$ qubits:
\begin{itemize}
    \item Qubits 1 to $n$: target state $\ket{\phi_u}$,
    \item Qubits $n+1$ to $2n$: candidate state $\ket{\psi}$,
    \item Qubit 0: ancilla for control-SWAP and measurement.
\end{itemize}
After each evaluation, only the candidate qubits and ancilla are reset for reuse.

\subsection{Gradient-Based Method: Neural Network Generator}
We implement a deep neural network $\mathcal{F}_\theta$ trained to output a normalized complex state vector $\ket{\psi} \in \mathbb{C}^{2^n}$ from a latent input $z \in \mathbb{R}^{256}$. The output is loaded into the circuit using Mottonen’s method via \texttt{qml.StatePrep}.

To enable gradient-based training despite non-differentiability, we implement a finite-difference autograd wrapper, \texttt{SwapTestFunction}, which approximates gradients during backpropagation.

\textbf{Architecture:} Six fully connected layers with GELU activation (except output). Training uses the Adam optimizer with learning rate $1 \times 10^{-4}$, and loss $\mathcal{L} = 1 - F$.

\textbf{Training Loop:} At each epoch, the model generates a candidate state, computes fidelity, and updates weights. Training stops early if fidelity $\sim 1.0$ is achieved.

\subsection{Gradient-Free Method: Evolutionary Strategy (QESwap)}
To reduce sensitivity to gradient noise and hyperparameter tuning, we implement QESwap, an evolutionary strategy that optimizes a parameter vector $w \in \mathbb{R}^{2\cdot 2^n}$ representing real and imaginary parts of the candidate state.

In each iteration:
\begin{itemize}
    \item $N=50$ candidates $\mathbf{w}_i = \mathbf{w} + \sigma \mathbf{z}_i$ are generated via Gaussian noise,
    \item Candidates are normalized and converted to quantum states,
    \item Fidelity is measured, and standardized advantages $A_i$ computed,
    \item Parameters are updated as $\mathbf{w} \gets \mathbf{w} + \frac{\alpha}{N \sigma} \sum_i A_i \mathbf{z}_i$.
\end{itemize}
This continues until fidelity exceeds a threshold or the maximum iteration count is reached.

\subsection{Experimental Protocol}
We evaluate both methods across 1–6 qubit systems over 1000 trials per configuration. Experiments are conducted in both noiseless and noisy simulators; real hardware evaluations are restricted to single-qubit reconstructions. Fidelity thresholds ($F \geq 0.95$ or $F \geq 0.99$) and convergence epochs are recorded.

\subsection{Snapshots at Multiple Points}
QSDC supports mid-circuit state reconstruction at arbitrary locations (Fig.~\ref{fig:quantum_bank}), enabling debugging, introspection, or reuse of intermediate quantum states.

\subsection{Quantum-Centric Hardware Requirements}
Realizing QSDC on hardware requires close coupling between classical and quantum processors (Fig.~\ref{fig:Q_C_arch}). Fast classical feedback enables model updates between mid-circuit measurements. This necessitates low-latency controllers, mid-circuit reset, and dynamic preparation—all features emerging in current SDKs like IBM’s dynamic circuits~\cite{IBMQuantumCentric2024}.

\subsection{State Deposition and Withdrawal}
Once high-fidelity estimates of quantum states are achieved, their corresponding complex-valued vectors are stored classically. When needed, these vectors are re-prepared on a quantum device via standard state preparation methods, enabling non-destructive memory and reuse of quantum states in dynamic circuits or QRAM workflows.


==> related_work_memory.tex <==
% \begin{table}[]
% \begin{tabular}{cl|c|ccccc}
% \multicolumn{2}{c|}{\textbf{Metric}}                                                                                                            & \textbf{QMB} & \textbf{Liu, et al \{{[}\}1\{{]}\}} & \textbf{Ahmed, et al \{{[}\}2\{{]}\}} & \textbf{Quek, et al \{{[}\}4\{{]}\}} & \textbf{Luu, et al \{{[}\}5\{{]}\}} & \textbf{Lange, et al \{{[}\}6\{{]}\}} \\ \hline
% \multicolumn{2}{c|}{\textbf{State Preservation}}                                                                                                & 0            & x                                   & x                                     & x                                    & x                                   & x                                     \\ \hline
% \multicolumn{2}{c|}{\textbf{Hardware Agnostic}}                                                                                                 & 0            & 0                                   & x                                     & 0                                    & x                                   & x                                     \\ \hline
% \multicolumn{2}{c|}{\textbf{Dataset Requirement}}                                                                                               & x            & x                                   & 0                                     & 0                                    & 0                                   & 0                                     \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Noiseless\\ Simulation\end{tabular}}}} & \textbf{Min. Fidelity Achieved} & 0.999        & 0.991                               & 0.9                                   & 0.999                                & 0.97                                & 0.956                                 \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                                                                         & \textbf{\# Epochs}              & 39           & 240                                 & 1000                                  & NA                                   & 1300                                & 1000                                  \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Noisy\\ Simulation\end{tabular}}}}     & \textbf{Min. Fidelity Achieved} & 0.99         & 0.99                                & x                                     & x                                    & 0.3                                 & 0.9093                                \\ \cline{2-8} 
% \multicolumn{1}{c|}{}                                                                                         & \textbf{\# Epochs}              & xyz          & xyz                                 & x                                     & x                                    & 1300                                & 1000                                  \\ \hline
% \multicolumn{2}{c|}{\textbf{Hardware Result}}                                                                                                   & 0            & x                                   & x                                     & x                                    & x                                   & x                                     \\ \hline
% \end{tabular}
% \end{table}


\begin{table*}[t!]
\centering
\fontsize{8.0pt}{9.5pt}\selectfont
\caption{Comparative Evaluation of the Quantum Memory Bank Architecture (QMBA) and Prior Quantum State Reconstruction Methods}
\begin{tabular}{cl||c|ccccc}
\multicolumn{2}{c||}{\textbf{Metric}}                                                                                                            & \textbf{QSDC} & \textbf{Liu, et al~\cite{liu_variational_2020}} & \textbf{Ahmed, et al~\cite{ahmed_quantum_2021}} & \textbf{Quek, et al~\cite{quek_adaptive_2018}} & \textbf{Luu, et al~\cite{luu_universal_2024}} & \textbf{Lange, et al~\cite{lange_adaptive_2023}} \\ \hline \hline
\multicolumn{2}{c||}{\textbf{State Preservation}}                                                                                                & \ding{51}            & \ding{55}                           & \ding{55}                             & \ding{55}                            & \ding{55}                           & \ding{55}                             \\ \hline
\multicolumn{2}{c||}{\textbf{Hardware Agnostic}}                                                                                                 & \ding{51}            & \ding{51}                           & \ding{55}                             & \ding{51}                            & \ding{55}                           & \ding{55}                             \\ \hline
\multicolumn{2}{c||}{\textbf{Dataset Requirement}}                                                                                               & \ding{55}            & \ding{55}                           & \ding{51}                             & \ding{51}                            & \ding{51}                           & \ding{51}                             \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Noiseless\\ Simulation\end{tabular}}}} & \textbf{Min. Fidelity Achieved} & $0.999$        & $0.991$                       & $0.9$                           & $0.999$                        & $0.97$                        & $0.956$                         \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                         & \textbf{\# Training Epochs}              & $5$           & $240$                         & $1000$                          & \texttt{NA}                           & $1300$                        & $1000$                          \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Noisy\\ Simulation\end{tabular}}}}     & \textbf{Min. Fidelity Achieved} & $0.996$         & \ding{55}                        & \ding{55}                             & \ding{55}                            & $0.3$                         & $0.9093$                        \\ \cline{2-8} 
\multicolumn{1}{c|}{}                                                                                         & \textbf{\# Training Epochs}              & $5$          & \ding{55}                         & \ding{55}                             & \ding{55}                            & $1300$                        & $1000$                          \\ \hline
\multicolumn{2}{c||}{\textbf{Quantum Hardware Result}}                                                                                                   & \ding{51}            & \ding{55}                           & \ding{55}                             & \ding{55}                            & \ding{55}                           & \ding{55}                             \\ \hline \hline
\end{tabular}
\label{tab:background_comparison}
\end{table*}



Recent years have seen the emergence of deep learning-based approaches to quantum state reconstruction and tomography methods~\cite{liu_variational_2020, ahmed_quantum_2021, gaikwad_gradient-descent_2025, quek_adaptive_2018, luu_universal_2024, lange_adaptive_2023}. However, these methods exhibit significant shortcomings. 
Table~\ref{tab:background_comparison} compares our proposed work QSDC against existing quantum state reconstruction and tomography methods. Our work is evaluated alongside prominent approaches by Liu et al.~\cite{liu_variational_2020}, Ahmed et al.~\cite{ahmed_quantum_2021}, Quek et al.~\cite{quek_adaptive_2018}, Luu et al.~\cite{luu_universal_2024}, and Lange et al.~\cite{lange_adaptive_2023}. Key metrics include state preservation, hardware agnosticism, dataset requirements, fidelity achieved under noiseless and noisy simulations, number of training epochs, and availability of hardware results. QSDC uniquely supports non-destructive state observation (state preservation), requires no training dataset, and achieves high fidelity with fewer epochs, even on real hardware, highlighting its practical efficiency and generalizability. While the table summarizes key methods in machine learning-based quantum state reconstruction, one approach ~\cite{gaikwad_gradient-descent_2025} has been excluded due to a fundamental incompatibility with the comparison criteria. Gaikwad et al.~\cite{gaikwad_gradient-descent_2025} employ the Uhlmann–Jozsa (UJ) fidelity as a loss function, under the assumption that the density matrix of the unknown quantum state is accessible. However, such access is fundamentally unavailable; indeed, the very motivation behind QST lies in the absence of this information. Consequently, using UJ fidelity in this context is not only impractical but infeasible to compute or implement on actual quantum hardware. As a result, we have excluded it from the comparative study.
The comparative analysis in Table~\ref{tab:background_comparison} highlights several key distinctions between our work, QSDC, and existing machine learning-based quantum state reconstruction methods. First and foremost, QSDC uniquely supports state preservation, enabling observation without collapsing the quantum state, an essential requirement for dynamic quantum computation. In contrast, all other methods in the comparison table rely on measurement-based approaches that inherently destroy the state, making them incompatible with mid-circuit observation or adaptive workflows. Additionally, QSDC is hardware agnostic, allowing seamless deployment across different quantum platforms. While some prior methods share this trait, others are constrained by specific hardware assumptions or simulation environments, for example, Ahmed et al.~\cite{ahmed_quantum_2021} present results exclusively on an optical system, limiting the generalizability of their approach. A significant advantage of QSDC is its independence from pre-collected datasets; it estimates quantum states in real time using a feedback-driven process rather than relying on large volumes of training data. This stands in contrast to all compared methods, which require curated datasets, typically from repeated measurements of identically prepared states, to learn state representations.
% 
% In terms of noiseless simulation fidelity, the QSDC achieves a high minimum fidelity of 0.999 in just 5 epochs, significantly outperforming several methods that require hundreds or even thousands of epochs to reach lower fidelity benchmarks\hl{comment on circuit size they considered compared to us}. The trend continues under noisy simulation conditions, where QSDC again achieves 0.99 fidelity, whereas the other methods either fail to report results or show considerable degradation in performance. Notably, hardware results are reported only for \hl{our work}, demonstrating its real-world feasibility, while all other works remain unvalidated on actual quantum devices. Taken together, these comparisons emphasize that \hl{the proposed method} not only offers theoretical advantages but also demonstrates superior empirical performance, making it a practical and scalable solution for non-destructive quantum state reconstruction.

==> results_noisemodel_snapshot.tex <==
\section{Noise Model} \label{noise_model}

To realistically simulate the behavior of near-term noisy quantum processors, we incorporate a detailed gate-level noise model derived from an IBM \texttt{GenericBackendV2} for the required number of qubits. This model is constructed using Qiskit's \texttt{NoiseModel} interface and imported into PennyLane via a custom Aer-based quantum device. The objective is to simulate realistic noise conditions akin to those found on current IBMQ hardware such as \texttt{ibmq\_quito} or \texttt{ibmq\_lima}.
\subsection{Basis Gate Set and Noisy Instructions}
The simulated device supports the following native basis gate set:
\(
\{\texttt{cx},\ \texttt{delay},\ \texttt{id},\ \texttt{measure},\ \texttt{reset},\ \texttt{rz},\ \texttt{sx},\ \texttt{x}\}
\)
Among these, the subset subject to explicit noise modeling includes:
\(
\{\texttt{id},\ \texttt{cx},\ \texttt{sx},\ \texttt{x},\ \texttt{measure}\}
\)
This configuration reflects real-device behavior where idle operations, entangling gates, and standard unitary rotations are affected by gate-dependent stochastic noise.
\subsection{Gate-Level Error Modeling}
To more accurately represent hardware-level fidelity degradation, the model includes the following calibrated error channels:

\begin{itemize}
    \item \textbf{Bit Flip Error:} Simulated using a Pauli-X channel with a probability \( p = 0.001 \), representing approximately 0.1\% chance of bit flips per gate operation.
    \item \textbf{Depolarizing Error:}
    \begin{itemize}
        \item Single-qubit gates: error probability = 0.002 (0.2\%)
        \item Two-qubit (CNOT) gates: error probability = 0.02 (2\%)
    \end{itemize}
    \item \textbf{Thermal Relaxation:}
    \begin{itemize}
        \item \( T_1 = 80\,\mu s \)
        \item \( T_2 = 100\,\mu s \)
        \item Gate time = \( 50\,\text{ns} \)
    \end{itemize}
\end{itemize}

The depolarizing and thermal relaxation errors are composed to create a composite noise model for CNOT gates. Single-qubit noise channels are applied to all instances of \texttt{rz}, \texttt{sx}, and \texttt{x} gates, and the bit-flip error is applied independently to capture additional stochastic behavior.

\subsection{Asymmetric and Hardware-Aware Modeling}

The noise model supports fine-grained control over the noise profile through Qiskit's \texttt{QubitChannel} abstraction, which uses Kraus operators to simulate stochastic error processes. Notable features include:

\begin{itemize}
    \item \textbf{Asymmetric noise} across different gate-qubit pairs to reflect hardware-specific non-uniformities.
    \item \textbf{Variable Kraus complexity}, with some \texttt{cx} gates represented by up to 16 Kraus operators, while simpler single-qubit gates use 3–4 operators.
\end{itemize}

This approach mirrors real IBMQ hardware behavior, capturing anisotropic and layout-specific noise behavior. For instance:

\begin{itemize}
    \item \texttt{cx}(0,1): \texttt{QubitChannel} with 16 Kraus operators
    \item \texttt{cx}(0,2): \texttt{QubitChannel} with 9 Kraus operators
\end{itemize}

%\subsection{Summary of Noise Parameters}

\begin{table}[h!]
\centering
\caption{Realistic Parameters Used in the Noise Model}
\begin{tabular}{c||cc}
% \hline
\textbf{Parameter} & \textbf{Value} & \textbf{Description} \\
\hline \hline
Bit flip probability (X) & 0.001 & Pauli-X error per gate \\
Single-qubit depolarizing error & 0.002 & For \texttt{rz}, \texttt{sx}, \texttt{x} \\
Two-qubit depolarizing error & 0.02 & For \texttt{cx} gates \\
$T_1$ & $80\,\mu s$ & Relaxation time \\
$T_2$ & $100\,\mu s$ & Dephasing time \\
Gate time & $50\,ns$ & Duration for gate operation \\
Kraus operators (\texttt{cx}(0,1)) & 16 & High noise interaction \\
Kraus operators (\texttt{cx}(0,2)) & 9 & Lower or different topology \\
\hline \hline
\end{tabular}
\label{tab:noiseparams}
\end{table}

\subsection{Effect on Simulation}

This detailed noise model was integrated into both the training and evaluation phases of our quantum state reconstruction framework. By emulating realistic gate-dependent and hardware-informed noise processes, we ensure that our fidelity metrics---particularly those derived from dot product overlap and SWAP test comparisons---accurately reflect the limitations and characteristics of real quantum hardware. This alignment is essential for validating the practical deployability of the reconstructed quantum states on NISQ-era processors.



==> table_big_state.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\label{tab:table_big_state}
\begin{table*}[]
\centering
\caption{Maximum fidelity attained and epochs taken to reach it for selected standard 1, 2, and 3 qubit quantum states}
\fontsize{7.0pt}{9.5pt}\selectfont
\begin{tabular}{cc|cccccccc|cccccccc}
\hline
\multicolumn{2}{c|}{\multirow{4}{*}{\textbf{Standard Quantum States}}}                                                                                                                                                                                                                               & \multicolumn{8}{c|}{\textbf{Noiseless Simulations}}                                                                                                                                                  & \multicolumn{8}{c}{\textbf{Noisy Simulations}}                                                                                                                                                      \\ \cline{3-18} 
\multicolumn{2}{c|}{}                                                                                                                                                                                                                                                                       & \multicolumn{4}{c|}{\textbf{Gradient Based (NN)}}                                                       & \multicolumn{4}{c|}{\textbf{Gradient Free (ES)}}                                           & \multicolumn{4}{c|}{\textbf{Gradient Based (NN)}}                                                       & \multicolumn{4}{c}{\textbf{Gradient Free (ES)}}                                           \\ \cline{3-18} 
\multicolumn{2}{c|}{}                                                                                                                                                                                                                                                                       & \multicolumn{2}{c|}{\textbf{State Vec.}}           & \multicolumn{2}{c|}{\textbf{Unitary}}              & \multicolumn{2}{c|}{\textbf{State Vec.}}           & \multicolumn{2}{c|}{\textbf{Unitary}} & \multicolumn{2}{c|}{\textbf{State Vec.}}           & \multicolumn{2}{c|}{\textbf{Unitary}}              & \multicolumn{2}{c|}{\textbf{State Vec.}}           & \multicolumn{2}{c}{\textbf{Unitary}} \\ \cline{3-18} 
\multicolumn{2}{c|}{}                                                                                                                                                                                                                                                                       & \textbf{\# E} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# E} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# E} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# E}     & \textbf{Fid.}     & \textbf{\# E} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# E} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# E} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# E}     & \textbf{Fid.}    \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{1 Qubit}}}  & $\bm{|0\rangle}$, $\bm{|1\rangle}$                                                                                                                                                                                                & 4             & \multicolumn{1}{c|}{0.99}          & 32            & \multicolumn{1}{c|}{0.99}          & 4             & \multicolumn{1}{c|}{0.99}          & 8                 & 0.99              & 28            & \multicolumn{1}{c|}{0.99}          & 39            & \multicolumn{1}{c|}{0.74}          & 5             & \multicolumn{1}{c|}{0.99}          & 60                & 0.99             \\ \cline{2-2}
\multicolumn{1}{c|}{}                                   & $\bm{|+\rangle}$, $\bm{|-\rangle}$                                                                                                                                                                                                & 4             & \multicolumn{1}{c|}{0.99}          & 32            & \multicolumn{1}{c|}{0.99}          & 4             & \multicolumn{1}{c|}{0.99}          & 9                 & 0.99              & 29            & \multicolumn{1}{c|}{0.99}          & 41            & \multicolumn{1}{c|}{0.75}          & 5             & \multicolumn{1}{c|}{0.99}          & 61                & 0.99             \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{2 Qubits}}} & $\bm{|00\rangle}$, $\bm{|01\rangle}$, $\bm{|10\rangle}$, $\bm{|11\rangle}$                                                                                                                                                        & 10            & \multicolumn{1}{c|}{0.99}          & 48            & \multicolumn{1}{c|}{0.99}          & 6             & \multicolumn{1}{c|}{0.99}          & 10                & 0.99              & 75            & \multicolumn{1}{c|}{0.98}          & 125           & \multicolumn{1}{c|}{0.61}          & 8             & \multicolumn{1}{c|}{0.99}          & 108               & 0.40             \\ \cline{2-2}
\multicolumn{1}{c|}{}                                   & $\bm{|\Phi^+\rangle}$, $\bm{|\Phi^-\rangle}$, $\bm{|\Psi^+\rangle}$, $\bm{|\Psi^-\rangle}$                                                                                                                                        & 12            & \multicolumn{1}{c|}{0.99}          & 50            & \multicolumn{1}{c|}{0.99}          & 7             & \multicolumn{1}{c|}{0.99}          & 12                & 0.99              & 77            & \multicolumn{1}{c|}{0.97}          & 123           & \multicolumn{1}{c|}{0.60}          & 9             & \multicolumn{1}{c|}{0.99}          & 110               & 0.41             \\ \hline
\multicolumn{1}{c|}{\textbf{3 Qubits}}                  & \begin{tabular}[c]{@{}c@{}}$\bm{\text{GHZ}_0^+}$, $\bm{\text{GHZ}_0^-}$, $\bm{\text{GHZ}_1^+}$, $\bm{\text{GHZ}_1^-}$, \\ $\bm{\text{GHZ}_2^+}$, $\bm{\text{GHZ}_2^-}$, $\bm{\text{GHZ}_3^+}$, $\bm{\text{GHZ}_3^-}$\end{tabular} & 18            & \multicolumn{1}{c|}{0.99}          & 76            & \multicolumn{1}{c|}{0.99}          & 13            & \multicolumn{1}{c|}{0.99}          & 21                & 0.99              & 84            & \multicolumn{1}{c|}{0.92}          & 93            & \multicolumn{1}{c|}{0.34}          & 26            & \multicolumn{1}{c|}{0.99}          & 20                & 0.15             \\ \hline
\end{tabular}
\label{tab:quantum_state_result}
\end{table*}






% \begin{table*}[]
% \centering
% \caption{Quantum States Results}
% \fontsize{7.0pt}{9.5pt}\selectfont
% \begin{tabular}{cc|cccccccc|cccccccc}
% \hline
% \multicolumn{2}{c|}{\multirow{4}{*}{\textbf{Quantum States}}}                                                                              & \multicolumn{8}{c|}{\textbf{Noiseless Simulations}}                                                                                                                                                     & \multicolumn{8}{c}{\textbf{Noisy Simulations}}                                                                                                                                                         \\ \cline{3-18} 
% \multicolumn{2}{c|}{}                                                                                                                      & \multicolumn{4}{c|}{\textbf{Gradient Based (NN)}}                                                         & \multicolumn{4}{c|}{\textbf{Gradient Free (ES)}}                                            & \multicolumn{4}{c|}{\textbf{Gradient Based (NN)}}                                                         & \multicolumn{4}{c}{\textbf{Gradient Free (ES)}}                                            \\ \cline{3-18} 
% \multicolumn{2}{c|}{}                                                                                                                      & \multicolumn{2}{c|}{\textbf{State Vector}}          & \multicolumn{2}{c|}{\textbf{Unitary}}               & \multicolumn{2}{c|}{\textbf{State Vector}}          & \multicolumn{2}{c|}{\textbf{Unitary}} & \multicolumn{2}{c|}{\textbf{State Vector}}          & \multicolumn{2}{c|}{\textbf{Unitary}}               & \multicolumn{2}{c|}{\textbf{State Vector}}          & \multicolumn{2}{c}{\textbf{Unitary}} \\ \cline{3-18} 
% \multicolumn{2}{c|}{}                                                                                                                      & \textbf{\# Ep} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# Ep} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# Ep} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# Ep}     & \textbf{Fid.}    & \textbf{\# Ep} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# Ep} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# Ep} & \multicolumn{1}{c|}{\textbf{Fid.}} & \textbf{\# Ep}    & \textbf{Fid.}    \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{1 Qubit}}}  & $\bm{|0\rangle}$                                                                 & 4              & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|1\rangle}$                                                                 & 4              & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|+\rangle} = \frac{1}{\sqrt{2}}   (\bm{|0\rangle} + \bm{|1\rangle})$        & 4              & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|-\rangle} = \frac{1}{\sqrt{2}}   (\bm{|0\rangle} - \bm{|1\rangle})$        & 5              & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\ \hline
% \multicolumn{1}{c|}{\multirow{8}{*}{\textbf{2 Qubits}}} & $\bm{|00\rangle}$                                                                & 9              & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|01\rangle}$                                                                & 11             & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|10\rangle}$                                                                & 7              & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|11\rangle}$                                                                & 11             & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|\Phi^+\rangle} = \frac{1}{\sqrt{2}}   (\bm{|00\rangle} + \bm{|11\rangle})$ & 12             & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|\Phi^-\rangle} = \frac{1}{\sqrt{2}}   (\bm{|00\rangle} - \bm{|11\rangle})$ & 12             & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|\Psi^+\rangle} = \frac{1}{\sqrt{2}}   (\bm{|01\rangle} + \bm{|10\rangle})$ & 12             & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\
% \multicolumn{1}{c|}{}                                   & $\bm{|\Psi^-\rangle} = \frac{1}{\sqrt{2}}   (\bm{|01\rangle} - \bm{|10\rangle})$ & 12             & \multicolumn{1}{c|}{0.99}          & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd                & tbd              & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd            & \multicolumn{1}{c|}{tbd}           & tbd               & tbd              \\ \hline
% \end{tabular}
% \label{tab:quantum_state_result}
% \end{table*}

==> todo.tex <==
%to do
1. Results for known states. 
2. Write explaining the figures in methods
% 5. SHow how generated states evolve over training iteration. Use Bloch sphere for demonstration. 
% 6. How much time is needed to reconstruct a state reliably? time vs reliability (with 1signma , 2 sigma etc. ) if the reconstruction time small enough to hold for decoherence time
% 7. How many copies are needed? How many shots reqd? relation to decoherence time
Per epoch time

# Add noisy bad results which shows noise affects 
